Learning-Based View Synthesis for Light Field Cameras

With the introduction of consumer light field cameras, light field imaging has recently become widespread. However, there is an inherent trade-off between the angular and spatial resolution, and thus, these cameras often sparsely sample in either spatial or angular domain. In this paper, we use machine learning to mitigate this trade-off. Specifically, we propose a novel learning-based approach to synthesize new views from a sparse set of input views. We build upon existing view synthesis techniques and break down the process into disparity and color estimation components. We use two sequential convolutional neural networks to model these two components and train both networks simultaneously by minimizing the error between the synthesized and ground truth images. We show the performance of our approach using only four corner sub-aperture views from the light fields captured by the Lytro Illum camera. Experimental results show that our approach synthesizes high-quality images that are superior to the state-of-the-art techniques on a variety of challenging real-world scenes. We believe our method could potentially decrease the required angular resolution of consumer light field cameras, which allows their spatial resolution to increase.

==> Discussion.tex <==
\begin{figure}[t]
\centering
\ifx\ShowTempImages\undefined
	\includegraphics[width=\linewidth]{Images/DepthComparison}
\else
	\includegraphics[width=\linewidth]{Images/DepthComparison_PlaceHolder}
\fi
\caption{\label{fig:DepthComp}
We compare our estimated disparity with other approaches. The darker color indicates regions that are closer to the camera. Although some of the other techniques produce disparity with higher quality than ours, they are often inaccurate around the occlusion boundaries. Our approach produces a reasonable disparity and is more accurate in the occlusion boundaries which are important regions for view synthesis.}
\end{figure}


\begin{figure}[!ht]
\centering
\ifx\ShowTempImages\undefined
	\includegraphics[width=\linewidth]{Images/ColorPredictorEval}
\else
	\includegraphics[width=\linewidth]{Images/ColorPredictorEval_PlaceHolder}
\fi
\caption{\label{fig:ColEstEval}
We evaluate the effect of our color predictor network. At the top, we show an inset of the {\sc Flower 1} scene containing a leave in the foreground covering part of a tree trunk in the background. At the bottom, we show an inset of the {\sc Cars} scene. Although our disparity captures the boundaries correctly, some of the warped images contain invalid information because of occlusion. For example, since the occlusion is vertical at the top set, the warped images from the left views contain artifacts, as shown by the red arrows. Our color predictor network produces high-quality results by collecting appropriate information from all the warped images. 
}
\end{figure}


\begin{figure}[!ht]
\centering
\ifx\ShowTempImages\undefined
	\includegraphics[width=\linewidth]{Images/FailureCase}
\else
	\includegraphics[width=\linewidth]{Images/FailureCase_PlaceHolder}
\fi
\caption{\label{fig:Failure}
Our approach fails to correctly estimate the disparity in the area between the leaves. In this case, none of the warped images have the post in between the leaves as can be seen in the ground truth image. Since our color predictor estimates the final image from these warped images, it fails to produce high quality image. However, our result is still more plausible than other methods.}
\end{figure}


\section{Discussion}
\label{sec:Discussion}

We begin the discussion by analyzing the effect of each component in our system. Fig.~\ref{fig:DepthComp} compares our estimated disparity against other approaches for the {\sc Seahorse} scene. Although the disparities produced by some of the other approaches have higher quality than ours, their disparity often has artifacts around the occlusion boundaries which are the most important regions for view synthesis. For example, none of the competing methods are able to appropriately estimate the disparity of the background at the middle of the green inset, or the boundaries of the seahorse snout in the red inset. As a result, these approaches often produce tearing artifact in these regions which can be seen in our supplementary video. 

Our method, on the other hand, can produce a reasonable disparity in these regions. Note that our method does not always produce accurate disparity, however, our inaccuracies usually happen in the regions that are not important for view synthesis. For example, part of the seahorse snout is incorrectly detected as background in our disparity (white region in left part of the red inset). However, this is a constant color region, and thus, this inaccuracy does not affect the quality of the synthesized results (see Fig.~\ref{fig:Motivation}). The main reason is that we train our disparity estimator network by directly minimizing the error between the synthesized and ground truth images. In the future, it would be interesting to combine our learning scheme with the ideas from the existing disparity estimation approaches to generate a more accurate disparity.


Next, we evaluate the effect of our color predictor network in Fig.~\ref{fig:ColEstEval}. In our approach, we use the estimated disparity at the novel view to warp all the input views to the novel view. As shown, these warped images often contain artifacts because of occlusion. Our color predictor network properly detects these regions and produces a high-quality image by collecting appropriate information from the warped images.

It is worth noting that since we use all the input views to generated the novel views, our results are generally less noisy comparing to the ground truth images. We refer the readers to our supplementary video to see this effect.This could be potentially useful for capturing light fields in low light conditions where noise is an issue.

Finally, our color predictor network generates the final image using the warped images. Therefore, in cases where none of the warped images contain valid information our approach is not able to produce high-quality results. One of such cases is shown in Fig.~\ref{fig:Failure} where our approach fails to synthesize the post in between the leaves and produces tearing artifacts. However, our synthesized image is considerably better than other approaches. 





==> Implementation.tex <==
\section{Implementation details}
\label{sec:Implementation}

To train these two networks efficiently, we propose to perform it in three stages by pre-training each network separately and then refining both networks simultaneously.

To train the disparity estimator network, we simply use the output of the network to warped one of the light field images to the novel view. The warped image can then be compared to the ground truth and the error can be backpropagated to update the network. We continue training this network until convergence.

Once the first stage is done we use the trained disparity estimator to generate training data for the second stage. To do this we use the disparity estimator network to produce disparity on the training data. These disparities as well as the warped images and the position of the novel view is fed into the quality estimator network. The network simply estimates the quality of the warped images which can then be used to generate the final image. This final image is compared to the ground truth and the error is backpropagated to update the weights of the quality estimator network.

Although the trained networks at this stage work reasonably well, we will still get benefit from refining these networks by training both of them at the same time. This is due to the fact that the disparity estimator has been forced to estimate depth even in the occluded regions. However, those regions could be handled by the quality estimator. By training both networks simultaneously, the networks would have connection which improves the quality of the results.


